Learning to Classify and Imitate Trading Agents in Continuous Double Auction Markets

Continuous double auctions such as the limit order book employed by exchanges are widely used in practice to match buyers and sellers of a variety of financial instruments. In this work, we develop an agent-based model for trading in a limit order book and show (1) how opponent modelling techniques can be applied to classify trading agent archetypes and (2) how behavioural cloning can be used to imitate these agents in a simulated setting. We experimentally compare a number of techniques for both tasks and evaluate their applicability and use in real-world scenarios.

==> preamble.tex <==
\usepackage{physics}

\makeatletter
\newif\if@restonecol
\makeatother
\let\algorithm\relax
\let\endalgorithm\relax
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{caption}

\makeatletter
\newcommand{\RemoveAlgoNumber}{\renewcommand{\fnum@algocf}{\AlCapSty{\AlCapFnt\algorithmcfname}}}
\newcommand{\RevertAlgoNumber}{\algocf@resetfnum}
\makeatother


%%% Commands

%% Math
\newcommand{\quaddist}{\ensuremath\operatorname{UQuadratic}}
\newcommand{\udist}{\ensuremath\operatorname{Uniform}}
\newcommand{\bernoulli}{\ensuremath\operatorname{Bernoulli}}
\newcommand{\expodist}{\ensuremath\operatorname{Exponential}}

%% agent functions

\newcommand{\wakeup}{\ProgSty{wakeup\_at}}
\newcommand{\marketorder}{\ProgSty{place\_market\_order}}
\newcommand{\limitorder}{\ProgSty{place\_limit\_order}}
\newcommand{\validtime}{\ProgSty{is\_valid\_time}}
\newcommand{\simrunning}{\ProgSty{sim\_running}}
\newcommand{\marketopen}{\ProgSty{market\_open}}
\newcommand{\bestbid}{\ProgSty{get\_best\_bid}}
\newcommand{\bestask}{\ProgSty{get\_best\_ask}}
\newcommand{\cancelorders}{\ProgSty{cancel\_all\_orders}}
\newcommand{\transactedvolume}{\ProgSty{get\_transacted\_volume}}
\newcommand{\buyvolume}{\ProgSty{get\_buy\_volume}}
\newcommand{\sellvolume}{\ProgSty{get\_sell\_volume}}
\newcommand{\currenttime}{\ProgSty{current\_time}}
\newcommand{\inventory}{\ProgSty{inventory}}
